Upper and Lower Bounds on the Smoothed Complexity of the Simplex Method

The simplex method for linear programming is known to be highly efficient in practice, and understanding its performance from a theoretical perspective is an active research topic. The framework of smoothed analysis, first introduced by Spielman and Teng (JACM '04) for this purpose, defines the smoothed complexity of solving a linear program with $d$ variables and $n$ constraints as the expected running time when Gaussian noise of variance $\sigma^2$ is added to the LP data. We prove that the smoothed complexity of the simplex method is $O(\sigma^{-3/2} d^{13/4}\log^{7/4} n)$, improving the dependence on $1/\sigma$ compared to the previous bound of $O(\sigma^{-2} d^2\sqrt{\log n})$. We accomplish this through a new analysis of the \emph{shadow bound}, key to earlier analyses as well. Illustrating the power of our new method, we use our method to prove a nearly tight upper bound on the smoothed complexity of two-dimensional polygons. We also establish the first non-trivial lower bound on the smoothed complexity of the simplex method, proving that the \emph{shadow vertex simplex method} requires at least $\Omega \Big(\min \big(\sigma^{-1/2} d^{-1/2}\log^{-1/4} d,2^d \big) \Big)$ pivot steps with high probability. A key part of our analysis is a new variation on the extended formulation for the regular $2^k$-gon. We end with a numerical experiment that suggests this analysis could be further improved.

==> figs/tikz_file/det-dist.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da601159494474153] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (329.04,218.1) -- (296.21,211.32) ;
\draw [shift={(331,218.5)}, rotate = 191.67] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da16736332779785668] 
\draw    (256.86,63.41) -- (448,189) ;
%Shape: Parallelogram [id:dp029836882863379488] 
% [color={rgb, 255:red, 65; green, 117; blue, 5 }
\draw  [draw opacity=0][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=0.18 ] (203.78,91.76) -- (407.06,137.08) -- (297.88,212.07) -- (94.61,166.75) -- cycle ;
%Straight Lines [id:da1500138763319412] 
\draw    (256.86,63.41) -- (315.2,278.15) ;
%Straight Lines [id:da601483538224197] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (377.5,228.5) -- (183,186.5) ;
%Straight Lines [id:da6958390303159552] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (296.21,211.32) -- (387,149.67) ;
\draw [shift={(387,149.67)}, rotate = 325.82] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(296.21,211.32)}, rotate = 325.82] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da2936586396129306] 
\draw    (256.86,63.41) -- (149.93,241.15) ;
%Straight Lines [id:da3259773897357544] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (299.55,209.32) -- (387,149.67) ;
%Straight Lines [id:da3403685536850527] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (297.88,212.07) -- (285.01,234.03) ;
\draw [shift={(284,235.76)}, rotate = 300.37] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da34888955494418983] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (387,149.67) -- (345.12,222.59) ;
\draw [shift={(345.12,222.59)}, rotate = 299.87] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (0,5.59) -- (0,-5.59)(10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(387,149.67)}, rotate = 119.87] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (0,5.59) -- (0,-5.59)(10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (221.38,219.07) -- (200.39,211.67) ;
\draw [shift={(198.5,211)}, rotate = 19.44] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (209.34,172.66) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ,rotate=-11.74] [align=left] {aff$\displaystyle ( F\cap W)$};
% Text Node
\draw (274,47) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q$};
% Text Node
\draw (123.7,152.12) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ,rotate=-11.74] [align=left] {$\displaystyle W$};
% Text Node
\draw (178.67,227.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle F$};
% Text Node
\draw (273.73,119.53) node [anchor=north west][inner sep=0.75pt]  [rotate=-343.64] [align=left] {$\displaystyle R$};
% Text Node
\draw (275.33,217.33) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle p$};
% Text Node
\draw (400.83,138.33) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle p'$};
% Text Node
\draw (335.73,101.53) node [anchor=north west][inner sep=0.75pt]  [rotate=-343.64] [align=left] {$\displaystyle R'$};
% Text Node
\draw (318.51,220.49) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ,rotate=-11.74] [align=left] {$\displaystyle s$$ $};
% Text Node
\draw (253.39,239.44) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=0] [align=left] {$\displaystyle \overline{\theta } \in W$$ $};
% Text Node
\draw (372.85,183.32) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-0] [align=left] {$\displaystyle \overline{\theta }^{\top }( p-p')$$ $};
% Text Node
\draw (210.39,224.44) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=0] [align=left] {$\displaystyle \theta $$ $};

\end{tikzpicture}

==> figs/tikz_file/dist-cone.tex <==
% Xinzhi: This tikz file is automatically generated by mathcha editor, link: https://www.mathcha.io/editor/Q2WoQCVmFEdfqZCK6qPjLteWJypziy9p08DSxMJpGM







\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da3592064404422608] 
\draw    (412.79,90.36) -- (185.5,236.07) ;
\draw [shift={(412.79,90.36)}, rotate = 147.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Straight Lines [id:da43460768159824315] 
\draw    (360.84,253.51) -- (185.5,236.07) ;
%Straight Lines [id:da47330666405551947] 
\draw    (360.84,253.51) -- (412.79,90.36) ;
%Straight Lines [id:da33505512651247993] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (319.28,214.52) -- (360.84,253.51) ;
%Straight Lines [id:da6293315142262832] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (319.28,214.52) -- (185.5,236.07) ;
%Straight Lines [id:da3841197178580813] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (319.28,214.52) -- (412.79,90.36) ;
%Shape: Triangle [id:dp6580362388605627] 
\draw  [draw opacity=0][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=0.2 ][dash pattern={on 0.84pt off 2.51pt}][line width=0.75]  (412.79,90.35) -- (319.15,251.32) -- (261.84,222.22) -- cycle ;
%Straight Lines [id:da35176801472255725] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (275.5,210) -- (291.89,236.01) ;
\draw [shift={(291.89,236.01)}, rotate = 57.77] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(275.5,210)}, rotate = 57.77] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Straight Lines [id:da3023467679043601] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (261.84,222.21) ;
\draw [shift={(261.84,222.21)}, rotate = 0] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Straight Lines [id:da6516884798943121] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (412.79,90.36) -- (261.84,222.21) ;
%Straight Lines [id:da6860175398716548] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (291.89,236.01) -- (261.84,222.22) ;
%Straight Lines [id:da24024023553342966] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (291.89,236.01) -- (412.79,90.36) ;

% Text Node
\draw (418.58,68.02) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (255.93,247.59) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle B$};
% Text Node
\draw (263.86,151.83) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle B'$};
% Text Node
\draw (300.11,229.26) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,xscale=1.1,yscale=1.1] [align=left] {$\displaystyle q$};
% Text Node
\draw (284.73,196.33) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,xscale=1.1,yscale=1.1] [align=left] {$\displaystyle \textcolor[rgb]{0.82,0.01,0.11}{q'}$};
% Text Node
\draw (243.62,207.15) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle \textcolor[rgb]{0.82,0.01,0.11}{x}$};
\draw (375,250) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle b_{d}$};


\end{tikzpicture}

==> figs/tikz_file/edgecounts.tex <==
% Xinzhi: This tikz file is automatically generated by mathcha editor, link: https://www.mathcha.io/editor/Q2WoQCVmFEdfqZCK6qPjLteWJypziy9p08DSxMJpGM

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da4824459250371491] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (428,139.8) -- (286,139.8) ;
\draw [shift={(286,139.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(428,139.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Straight Lines [id:da6240195953567047] 
\draw    (426,150.8) -- (288,150.8) ;
\draw [shift={(286,150.8)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(428,150.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da12589308806645683] 
\draw    (286,139.8) -- (286,158.8) ;
%Straight Lines [id:da7859420137066957] 
\draw    (428,139.8) -- (428,158.8) ;
%Straight Lines [id:da6380781281343051] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ]   (286,139.8) -- (208,198.8) ;
%Straight Lines [id:da42700562293346644] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (408,49.8) -- (286,139.8) ;
%Straight Lines [id:da9182056796383498] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (377.21,73.39) -- (426.79,138.22) ;
\draw [shift={(428,139.8)}, rotate = 232.59] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(376,71.8)}, rotate = 52.59] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da042755669299258114] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ]   (428,139.8) -- (486,183.8) ;
%Shape: Pie [id:dp41789800442100455] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=0 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.53 ] (305.65,126.11) .. controls (305.65,126.11) and (305.65,126.11) .. (305.65,126.11) .. controls (308.72,130.21) and (310.46,134.84) .. (310.93,139.43) -- (287.87,139.43) -- cycle ;
%Shape: Arc [id:dp14809945499425647] 
\draw  [draw opacity=0] (310.93,139.43) .. controls (310.9,133.89) and (308.63,128.93) .. (305.05,125.56) -- (293.93,139.54) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (310.93,139.43) .. controls (310.9,133.89) and (308.63,128.93) .. (305.05,125.56) ;  

% Text Node
\draw (210,146) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ,xscale=1.1,yscale=1.1] [align=left] {$\displaystyle e_I$};
% Text Node
\draw (351,153) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle \ell _{I^+}$};
% Text Node
\draw (435,130) node [anchor=north west][inner sep=0.75pt]  [xscale=1.1,yscale=1.1] [align=left] {$\displaystyle p_{I^+}$};
% Text Node
\draw (401,86) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,xscale=1.1,yscale=1.1] [align=left] {$\displaystyle \geq \gamma $};
% Text Node
\draw (233,102) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,xscale=1.1,yscale=1.1] [align=left] {$\displaystyle \theta _{I} \geq \gamma /\ell _{I^+}$};


\end{tikzpicture}
